Subject-driven Text-to-Image Generation via Apprenticeship Learning

Recent text-to-image generation models like DreamBooth have made remarkable progress in generating highly customized images of a target subject, by fine-tuning an ``expert model'' for a given subject from a few examples. However, this process is expensive, since a new expert model must be learned for each subject. In this paper, we present SuTI, a Subject-driven Text-to-Image generator that replaces subject-specific fine tuning with in-context learning. Given a few demonstrations of a new subject, SuTI can instantly generate novel renditions of the subject in different scenes, without any subject-specific optimization. SuTI is powered by apprenticeship learning, where a single apprentice model is learned from data generated by a massive number of subject-specific expert models. Specifically, we mine millions of image clusters from the Internet, each centered around a specific visual subject. We adopt these clusters to train a massive number of expert models, each specializing in a different subject. The apprentice model SuTI then learns to imitate the behavior of these fine-tuned experts. SuTI can generate high-quality and customized subject-specific images 20x faster than optimization-based SoTA methods. On the challenging DreamBench and DreamBench-v2, our human evaluation shows that SuTI significantly outperforms existing models like InstructPix2Pix, Textual Inversion, Imagic, Prompt2Prompt, Re-Imagen and DreamBooth, especially on the subject and text alignment aspects.

==> tables_and_figures/figure_data_collection.tex <==
\begin{figure}[!tbh]
    \centering
    \includegraphics[width=0.9\linewidth]{assets/introduction.001.jpeg}
    \caption{
        \small
        Details of the Data Collection Procedure
    }
    \label{fig:data_collection}
\end{figure}

==> tables_and_figures/figure_teaser_small.tex <==
\begin{figure}[!htb]
    \centering
    \vspace{-10mm}
    \includegraphics[width=1\textwidth]{assets/teaser.002}
    \vspace{-5mm}
    \caption{
    \small We train \emph{a single} {\modelname} \emph{model} to generate novel scenes faithfully reflecting given subjects (unseen in training, specified only by 3-5 in-context text$\to$image demonstrations), without any optimization.
    }
    \vspace{-2.5mm}
    \label{fig:teaser}
\end{figure}

